Game of Life on Graphs

We consider a specific graph dynamical system inspired by the famous Conway's Game of Life in this work. We study the properties of the dynamical system on different graphs and introduce a new efficient heuristic for graph isomorphism testing. We use the evolution of our system to extract features from a graph in a deterministic way and observe that the extracted features are unique and the distance induced by that features satisfy triangle inequality for all connected graphs with up to ten vertices.

==> scratch.tex <==
\section{Phase Transition}
\label{sec:phase}

Studying of phase transitions is a rich topic at the intersection of computer science and statistical physics. Random instances of many different problems and families of structures in computer science undergo a phase transition with respect to one or more parameters. Moreover, the most difficult and complex instances are observed around the transition point, while the instances far from the transition are usually simpler.

One of the first famous results on this topic was about 3-SAT phase transition \cite{3SAT}. In that seminal paper, authors consider random instances of the boolean satisfability problem with $N$ variables, $M$ clauses and $3$ variables per clause. For large enough values of $N$ (what is called thermodynamic limit in physics) the random instances undergo a sharp SAT-UNSAT phase transition with respect to density parameter $k = \frac{M}{N}$ at some value $k=\alpha$: for $k < \alpha-\epsilon$ random instances are satisfiable with probabiltiy one while for $k > \alpha+\epsilon$ random instances are unsatisfiable with probablity one.

\subsection{Transition of the Game}


\item Why the most complex dynamics exist around the $p = \frac{1}{n}$ transition point? What can the graph topology say about the dynamics of Game of Life and vice versa?



\begin{figure}[ht]
\centering
\includegraphics[width=0.33\textwidth]{pict/metrics/line1/6-0.png}\hfill
\includegraphics[width=0.33\textwidth]{pict/metrics/line1/6-28.png}\hfill
\includegraphics[width=0.33\textwidth]{pict/metrics/line1/6-92.png}
% Reduce the figure size so that it is slightly narrower than the column.
\caption{An example of a line in the space of all graphs with six vertices. The 'GLG'-distance between the first and thrid graphs equals the sum of the two other distances. The graph in the middle can be interpreted as the half sum of two other graphs.}
\label{fig:metric_line1}
\end{figure}





%__________________________________________________


In the Figure~\ref{fig:ex} we show an example of an evolution that starts {\it blinking} at step four and never dies. In Figures~\ref{fig:line0},\ref{fig:line1} we illustrate the Game of Life on line graph - in both cases the evolution {\it dies} in a few steps. 


\begin{figure}[ht!]
\centering
\includegraphics[width=0.25\textwidth]{pict/ex/p0.png}\hfill
\includegraphics[width=0.25\textwidth]{pict/ex/p1.png}\hfill
\includegraphics[width=0.25\textwidth]{pict/ex/p2.png}\hfill
\includegraphics[width=0.25\textwidth]{pict/ex/p1.png}
% Reduce the figure size so that it is slightly narrower than the column.
\caption{An exemplary Game of Life on a graph with five vertices. We start with the initial pattern on the left and proceed for three steps until the life pattern from the fourth step repeats the life pattern from the second step. Thus the complexity of this game equals three.}
\label{fig:ex}
\end{figure}


\begin{figure}[ht!]
\centering
\includegraphics[width=0.33\textwidth]{pict/line/l_00.png}\hfill
\includegraphics[width=0.33\textwidth]{pict/line/l_01.png}\hfill
\includegraphics[width=0.33\textwidth]{pict/line/l_02.png}
% Reduce the figure size so that it is slightly narrower than the column.
\caption{An exemplary Game of Life on a line graph with five vertices. We start with the initial pattern on the left and proceed for three steps until the game {\it dies} at the third step. Thus the complexity of this game equals two.}
\label{fig:line0}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.2\textwidth]{pict/line/l_10.png}\hfill
\includegraphics[width=0.2\textwidth]{pict/line/l_11.png}\hfill
\includegraphics[width=0.2\textwidth]{pict/line/l_12.png}\hfill
\includegraphics[width=0.2\textwidth]{pict/line/l_13.png}\hfill
\includegraphics[width=0.2\textwidth]{pict/line/l_02.png}
% Reduce the figure size so that it is slightly narrower than the column.
\caption{An exemplary Game of Life on a line graph with five vertices. We start with the initial pattern on the left and proceed for three steps until the game {\it dies} at the fifth step. Thus the complexity of this game equals four.}
\label{fig:line1}
\end{figure}
